A tunable macroscopic quantum system based on two fractional vortices

We propose a tunable macroscopic quantum system based on two fractional vortices. Our analysis shows that two coupled fractional vortices pinned at two artificially created \kappa\ discontinuities of the Josephson phase in a long Josephson junction can reach the quantum regime where coherent quantum oscillations arise. For this purpose we map the dynamics of this system to that of a single particle in a double-well potential. By tuning the \kappa\ discontinuities with injector currents we are able to control the parameters of the effective double-well potential as well as to prepare a desired state of the fractional vortex molecule. The values of the parameters derived from this model suggest that an experimental realisation of this tunable macroscopic quantum system is possible with today's technology.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v2.00 -- LaTeX macros for frequently used
%%% abbraviations
%%% Manipulated by Dennis Heim 14.08.2012, see {my} enviroment

\RequirePackage{xspace}

%stupid macros kike \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
%\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\xspace}
\newcommand{\rhs}{r.h.s.\xspace}


%units
\newcommand{\units}[1]{\ensuremath{\,\mathrm{#1}}}
%big \frac called \ratio
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp[n]{f}{x}
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}

%%
%% Freq used math symbols
%%

%Elliptic fns
%% \begin{my}
%% I removed \mathop \nolimits in following commands because they lower 
%% the symbols which looks ugly due to Prof. Schleich and Karl
%% Dennis Heim, 14.08.2012
\newcommand{\am}{\,{\mathrm{am}}}
\newcommand{\dn}{\,{\mathrm{dn}}}
\newcommand{\sn}{\,{\mathrm{sn}}}
\newcommand{\cn}{\,{\mathrm{cn}}}
\newcommand{\gd}{\,{\mathrm{gd}}}
\newcommand{\E} {\,{\mathrm{E}}}
\newcommand{\F} {\,{\mathrm{F}}}
\newcommand{\K} {\,{\mathrm{K}}}
\newcommand{\Heavyside}{\,{\mathrm{H}}}
\newcommand{\sgn}{\,{\mathrm{sgn}}}
%% \end{my}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
%\newcommand{\const}{\mathop{const}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}

%just shortcuts
\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%\iffalse%{
\RequirePackage{amssymb}

%Misc. macros to discuss with co-authors
\RequirePackage{changebar}
\newcommand{\X}[1]{}
%\newcommand{\Q}[1]{\cbstart {\small\sffamily Q: #1}\cbend}

\RequirePackage[normalem]{ulem}

\definecolor{uniorange}{RGB}{240, 100, 65}
\definecolor{gray}{rgb}{0.6,0.5,0.7}
\definecolor{darkgreen}{rgb}{0,.4,0}

\newcommand{\era}[1]{\textcolor{gray}{#1}}
\newcommand{\new}[1]{\textcolor{uniorange}{#1}}
\newcommand{\del}[1]{\textcolor{uniorange}{\sout{#1}}}
\newcommand{\chg}[1]{\textcolor{magenta}{#1}}
\newcommand{\KV}[1]{\textcolor{magenta}{#1}}


%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}



